Learning Robust Algorithms for Online Allocation Problems Using Adversarial Training

We address the challenge of finding algorithms for online allocation (i.e. bipartite matching) using a machine learning approach. In this paper, we focus on the AdWords problem, which is a classical online budgeted matching problem of both theoretical and practical significance. In contrast to existing work, our goal is to accomplish algorithm design {\em tabula rasa}, i.e., without any human-provided insights or expert-tuned training data beyond specifying the objective and constraints of the optimization problem. We construct a framework based on insights and ideas from game theory, adversarial training and GANs Key to our approach is to generate adversarial examples that expose the weakness of any given algorithm. A unique challenge in our context is to generate complete examples from scratch rather than perturbing given examples and we demonstrate this can be accomplished for the Adwords problem. We use this framework to co-train an algorithm network and an adversarial network against each other until they converge to an equilibrium. This approach finds algorithms and adversarial examples that are consistent with known optimal results. Secondly, we address the question of robustness of the algorithm, namely can we design algorithms that are both strong under practical distributions, as well as exhibit robust performance against adversarial instances. To accomplish this, we train algorithm networks using a mixture of adversarial and practical distributions like power-laws; the resulting networks exhibit a smooth trade-off between the two input regimes.

==> app-ski-rental.tex <==
\section{Additional plots for Ski Rental}
\label{app:ski-rental}

\begin{figure}[h]
  \begin{center}  
    \includegraphics[width=\textwidth]{figs/sr_cont_alg_behaviour.pdf}
    \caption{The learnt algorithm instantiated at various $(B,N)$ values as CDF of buying over time (blue curve). The orange x's correspond to the optimal strategy in each case.}
    \label{fig:continuousskirental_more}
  \end{center}
\end{figure}

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> asymptotic_skirental.tex <==
%Before applying the complete YaoGAN paradigm with two neural networks on the very difficult problem of fractional AdWords, we take smaller steps, and expand upon the previous simple example of ski rental. 

%In the previous example, we consider finding an algorithm of the ski rental problem for a fixed buying price $B$ and time horizon $N$.

Our goal here is to learn an algorithm that simultaneously captures the algorithms for all individual $B$ and $N$ values.  Note that we can no longer explicitly maintain and update the algorithms, one for each $B, N$, nor use exhaustive search to find best responses. Following the YaoGAN program, on the algorithm side, we train a deep neural network to represent the unified algorithm that takes $B$ can be instantiated to yield a specific algorithm for any given $B$ and $N$.  On the adversary side, we don't resort to a deep neural networks yet because the input space our algorithm network is still fairly straightforward, and simple methods are quite effective to come up with good responses for training.

We demonstrate the trained algorithm in Figure~\ref{fig:continuousskirental} by instantiating it at various values of $B$ and $N$. The result is very close to the optimal strategy in all cases, and indicates that our theoretical insights from Section~\ref{sec:MWU} largely extends to more general settings. We defer further details to Appendix~\ref{app:ski-rental}.

\begin{figure}[h]
\label{fig:continuousskirental}
  \begin{center}  
    \includegraphics[width=\textwidth]{figs/sr_cont_alg_behaviour_small.pdf}
    \caption{The meta-algorithm instantiated at various $(B,N)$ values as cdf of buying over time (blue curve). The orange x's correspond to the optimal strategy in each case.}
  \end{center}
\end{figure}


% As to the internal structure of the algorithm neural network, recall we want to learn a continuous distribution (over $[0,1]$) for every $\beta$. We use $50$ Gaussian kernels $N(x_i,\sigma)$ for $i=1,\ldots,50$ with fixed means (i.e., $x_i$'s equally spaced over $[0,1]$) and standard deviation $\sigma=2/50$, and take a weighted average of these Gaussian kernels as the distributions learned by our neural network. In particular, given any $(\alpha,\beta)$ as input, the neural network uses $\beta$ to derive weights $w_i$'s over the Gaussian kernels (where $\sum_i w_i=1$), and take the weighted sum of the c.d.f of these fixed Gaussian kernels at point $\alpha$ as the output of the algorithm.

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> broader-impact.tex <==
\bigskip
\noindent
\textbf{Statement of Broader Impact.}

\noindent
We believe this work is of mostly theoretical interest, in its current form. It is a framework to help in the discovery of theoretical worst-case or practically robust algorithms; as for any optimization framework or algorithm, it can be applied to domains of broader societal impact, but we do not contribute or foresee any such direct impact.

%We believe this work is of mostly theoretical interest: the prospect of gaining intuition about worst-case algorithms without any human-provided data is a captivating possibility. Our work is a first step in this direction. Even the part of the paper that seems most interesting to practitioners (robust stochastic training, or finding algorithms that perform well on practical distributions as well as adversarial shocks), most likely requires combining our ideas with a plethora of practical heuristics in order to design production-ready solutions. For these reasons, we do not expect this work to have significant broader societal impact within the foreseeable future.



==> intro.tex <==
\section{Introduction}
It has been a long-standing ambition of machine learning to learn from \emph{first principles}, that is, a machine learning program that learns \emph{without any human-provided data} beyond an appropriate definition of the task at hand~\citep{silver2018general}. The community has made impressive strides towards this goal in recent years, most notably in the domain of tabletop games such as chess, Go, shogi~\citep{silver2018general} and poker~\citep{brown2018superhuman}, where programs have been trained to play at superhuman levels without consuming any game-specific human expertise except, naturally, the rules of the game. 

In this work, we look at the task of using ML to \emph{design algorithms for optimization problems}. Similar to tabletop games, the task of algorithm design has succinct and well-defined objectives, so learning from first principles is potentially feasible. Moreover, the task is very intriguing as it typically requires a significant amount of time and expertise for humans to accomplish. If successful, such an approach can have impactful ramifications: researchers could accelerate the speed of discovery by offloading to machines the time-consuming process of finding problem-specific insights, which can be crucial in improving the state of the art for many problems both in theory and in practice.

A typical ML approach to algorithm design is to define a model that represents the space of possible algorithms and train the model against a pre-defined training set. The assumption is that the training set is carefully chosen to capture future input distributions well, so the learned algorithm generalizes to future inputs of interest. However, designing this distribution requires domain-specific knowledge and is incompatible with learning from first principles.

We take a different approach: train the algorithm against \emph{worst-case inputs}. In other words, the fitness of an algorithm is only as good as its fitness on the worst possible input. This conceptually removes the need for pre-defining a training set. Worst-case algorithm design is motivated by theoretical computer science (TCS) that traditionally considers algorithms with worst-case guarantees due to their robustness against arbitrary inputs.

There have been very few prior attempts at learning worst-case algorithms.
% Along the line of learning worst-case algorithms,
A particularly relevant result is by \cite{kong2018new} that uses reinforcement learning to learn theoretically optimal algorithms for online optimization problems. They show how to learn worst-case algorithms using a training set by introducing the notion of universal and high-entropy training sets. Roughly speaking, such a training set serves as a very effective benchmark in the sense that the task of finding an algorithm with strong worst-case guarantee reduces to finding an algorithm that performs well against this training set. Not surprisingly, for a given optimization problem, coming up with such a training set can require significant domain expertise a priori. In the current work, the goal is different: we aim to both provide a new technique for worst-case learning and leverage it to remove the need for a training set.

We utilize \emph{adversarial training}~\cite{GSS14,madry2018} as our main technique. Notably, our methods draw insights from game theory, analysis of algorithms, online learning and generative adversarial networks (GANs)~\cite{GAN}. This is in stark contrast to prior work that considers adversarial training through the lens of robust optimization. This alternative view of the technique might be of independent interest to the ML community.

On a high-level, the technique learns an algorithm iteratively: by considering the current version of the algorithm, finding its worst-case input (also called adversarial input, since one can imagine a hostile adversary hand-picking it), and optimizing the algorithm's response on this input. Naturally, finding the worst-case input is often a hard problem in itself. For simpler optimization problems, rudimentary strategies such as random search or grid search can provide a fairly effective adversary. For problems with more interesting underlying space, we propose a general framework that uses deep learning to both guide our search for worst-case inputs and optimize the algorithm. In other words, we propose an end-to-end ML framework that can be roughly separated into two components: the algorithm agent and the adversary. Their goals are to learn the optimal algorithm and a set of input instances that captures the essential difficulty of the given optimization problem, respectively. Similar to a generative adversarial network (GAN), we use two neural networks, one for the algorithm agent and another for the adversary. We start from scratch, train these two networks against each other, and let them evolve simultaneously. We call our framework \emph{YaoGAN} due to this structural similarity to GAN and the connection to Yao's classic Lemma (see Section~\ref{sec:Yao} for details).

In this initial effort, we follow \cite{kong2018new} in focusing on \emph{online optimization problems}~\citep{BN09} where each input is a sequence arriving over time, and the algorithm needs to make an immediate and irrevocable decision at each time step without knowing the future input.
%We further restrict our attention to problems that can be solved or approximated by algorithms requiring a small amount of memory. There are abundant well-studied and interesting problems bearing such properties in online optimization, typically when the structure of the problem exhibits certain Markov property so it is sufficient for the algorithm to maintain a succinct state capturing past information. 

We consider two online optimization problems, the \emph{ski rental} problem and the \emph{AdWords} problem. Ski rental~\citep{Karlin86} has been a staple introductory example in online analysis due to the simplicity of the statement and non-triviality of the optimal solution. We use a straightforward application of the adversarial training concept and demonstrate its viability for learning algorithms with worst-case guarantees by reconstructing the optimal textbook algorithm for the problem.

We evaluate the full YaoGAN framework on a harder, AdWords problem~\citep{MSVV07}---a well-known problem motivated by online advertising. The AdWords problem is of particular importance in the online advertising as it captures the question of allocation of ad slots arriving over time to advertisers with budget constraints. Furthermore, having a robust algorithm is very important in such a setting -- one may learn better performing policies for specific input distributions, but in reality, traffic patterns can change abruptly based on external events, and advertisers can change their bidding and targeting at any time. Besides the practical importance, the problem has also been of great interest in the online algorithms literature, being closely related to numerous variants of the online bipartite matching problem~\citep{Meh13}, which remains an actively studied area in algorithm design, for example in the setting of ride-sharing platforms~\citep{Dickerson17,AshlagiBDJSS19}. 

%For both of these problems, we have a good understanding of the structures inherent in optimal algorithms and difficult inputs, allowing us to evaluate the learned algorithms. 
Our experiments for this specific hard problem demonstrate that our framework can be effective at finding algorithms as well as difficult input instances that are consistent with optimal results. We believe further study along this direction can lead to more exciting developments.
We use generic neural network architecture and ML methods (e.g., Adam optimizer~\citep{kingma2014adam}) in our experiments, and do not optimize the training set-up or hyperparameters, since our focus in this paper is not in extending ML techniques, but in applying our high-level paradigm to learn algorithms from first principles. We believe the co-evolution of new ML techniques tailored to this task will be essential to the ultimate success of this approach. We leave that aspect, as well as the tantalizing question of applying the framework to solve open algorithm design problems, to future work. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In our context, the problem of learning algorithms from first principles is also related to an important issue in both ML and algorithms: what input instances is the learned algorithm expected to handle? The typical ML approach is to train the program against a pre-defined training set, with the assumption that the training set is carefully chosen to capture future input distributions well, so the learned algorithm generalizes to future input of interest. On the other hand, the algorithm design community in theoretical computer science (TCS) traditionally considers algorithms with worst-case guarantees due to their robustness against arbitrary inputs. Our aim is to initiate the learning of worst-case guarantees in the context of ML


% We argue that the standard approach often fails to find robust algorithms and propose a novel (in the context of ML) ``best-response learning'' paradigm that enables and stabilizes learning of worst-case algorithms.

% Along the line of learning worst-case algorithms, a particularly relevant result is by \cite{kong2018new} that uses reinforcement learning to learn theoretically optimal algorithms for online optimization problems, and one of the key ideas they introduce is the notion of universal and high-entropy training sets. Roughly speaking, such a training set serves as a very effective benchmark in the sense that the task of finding an algorithm with strong worst-case guarantee reduces to finding an algorithm that performs well against this training set. Not surprisingly, for a given optimization problem, coming up with such a training set can require significant domain expertise a priori. In the current work the goal is to go beyond the framework of universal training sets, and enable learning of algorithms without even this prior domain knowledge.

% To overcome this issue, we draw insights from the fields of game theory, analysis of algorithms, and online learning, as well as generative adversarial networks (GANs,~\citet{GAN}). In particular, we introduce a training framework that aims to learn a strong worst-case algorithm and an effective benchmark training set simultaneously, all without relying on any human domain expertise beyond specifying how to compute the objective of the optimization problem. If successful, such an approach would have impactful ramifications: researchers could accelerate the speed of discovery by offloading to machines the time-consuming process of finding problem-specific insights, which can be crucial in improving the state of the art for many problems both in theory and in practice.

% At the high level, our framework has two components: the algorithm agent and the adversary. Their goals are to learn the optimal algorithm and a set of input instances that captures the essential difficulty of the given optimization problem, respectively. For simple optimization problems, rudimentary strategies such as random search or grid search can provide a fairly effective adversary. For problems with more interesting underlying space, we exploit deep learning to guide our search for the distribution of difficult inputs. Similar to a generative adversarial network (GAN), we use two neural networks, one for the algorithm agent and another for the adversary. We start from scratch, train these two networks against each other, and let them evolve simultaneously. We call our program \emph{YaoGAN} due to this structural similarity to GAN and the connection to the classic Yao's Lemma (see Section~\ref{sec:Yao} for details); this is our main technical contribution.

% In this initial effort, we follow \cite{kong2018new} in focusing on online optimization problems~\citep{BN09} where each input is a sequence arriving over time, and the algorithm needs to make an immediate and irrevocable decision at each time step without knowing the future input. We further restrict our attention to problems that can be solved or approximated by algorithms requiring a small amount of memory. There are abundant well-studied and interesting problems bearing such properties in online optimization, typically when the structure of the problem exhibits certain Markov property so it is sufficient for the algorithm to maintain a succinct state capturing past information. 

% We consider two online optimization problems, the {\em ski rental\/} problem and the {\em fractional AdWords\/} problem. Ski rental~\citep{Karlin86} has been a staple introductory example in online analysis. The second problem, fractional AdWords~\citep{MSVV07}, is (a fractional relaxation of) a well-known problem motivated by online advertising. Moreover, the Adwords problem is closely related to numerous variants of the online bipartite matching problem, which is still an actively studied area in algorithm design, for example in the setting of ride-sharing platforms~\citep{Dickerson17,AshlagiBDJSS19}. For these problems, we have a good understanding of the structures of the optimal algorithm and difficult inputs, so we can verify that our paradigm leads to something meaningful. Our experiments, although fairly limited and preliminary, demonstrate that our framework can be effective at finding algorithms as well as difficult input instances that are consistent with optimal results. We believe further study along this direction can lead to more exciting developments.

% We use generic neural network architecture and ML methods (e.g., Adam optimizer~\citep{kingma2014adam}) in our experiments, and do not optimize the training set-up or hyperparameters, since our focus in this paper is not in extending ML techniques, but in applying our high-level paradigm to learn algorithms from first principles. We believe the co-evolution of new ML techniques tailored to this task will be essential to the ultimate success of this approach. We leave that aspect, as well as applying the framework to more open algorithm design problems, to future work. 

% %Note that we pick these well-studied problems to experiment because we can compare our findings against the known optimal algorithm and worst-case input distribution 

\noindent{\bf Related work.} The most relevant paper to ours is an approach by \cite{kong2018new} that uses reinforcement learning (RL) to find competitive algorithms for online optimization problems including the AdWords problem, online knapsack and the secretary problem. They introduce the notions of universal and high-entropy training set that are tailor-made to facilitate the convergence to worst-case competitive algorithm.  \cite{deudon2018learning} and \cite{kool2018attention} use RL to solve the traveling salesman problem (TSP) in the two-dimensional plane. Both uniformly sample the input points from the unit square and teach the network to optimize the expected performance on this input distribution without having access to exact solutions. Nevertheless, the learned algorithms from both approaches seem competitive with state-of-the-art methods, at least for modest input sizes. \cite{vinyals2015pointer} introduce the Pointer Network, a sequence-to-sequence model that successfully manages to approximately find convex hulls, Delaunay triangulations and near-optimal planar TSPs. They assume access to an exact solution and use supervised learning to train the model, while their input is uniformly sampled from the unit square. \cite{graves2014neural} introduce the Neural Turing machines, a differentiable and computationally universal Turing machine model, and use supervised learning to teach them basic algorithms such as copying or sorting. \cite{kaiser2015neural} introduce the parallel and computationally universal Neural GPU and use supervised learning to teach it addition and multiplication that seemingly generalizes to arbitrary lengths. 

We point out some other related results without going into details: the work of~\cite{bello2016neural} studies applying RL on combinatorial problems including TSP and Knapsack; the work of~\citet{Dai17} exploits embedding and RL to design heuristic algorithms for classic graph problems on specific distributions;~\citet{boutilier2016budget} uses RL to solve Budget Allocation problem;~\cite{Duetting0NPR19} applies deep learning techniques to designing incentive compatible auction mechanisms. Readers insterested in ski rental and AdWords can consult~\citet{Buchbinder:Naor:survey} and \citet{Meh13} for a more thorough coverage.

To the best of our knowledge, previous results mostly focus on the algorithm side, and either learn algorithms designed to work on specific input distributions of interest, or utilize supervised learning to mimic a known method, or (in the case of~\citet{kong2018new}) rely on domain expertise to provide hard input instances to train algorithms that are competitive in worst-case. We do not wish to detract from the value of optimizing an algorithm on a specific distribution if it is of special interest. Indeed, a practitioner optimizing for a distribution $\mc{D}$ could likely design algorithms that outperform classic solutions on $\mc{D}$ since classic solutions typically protect against worst-case inputs and might be overly pessimistic on $\mc{D}$. Our goal is different: facilitate the discovery of new algorithms with strong worst-case performance on open problems where we do not have a known difficult input distribution at hand. Such learned strategies could then potentially be later fine-tuned to adapt to specific input distributions, while retaining some worst case guarantees. We consider the results here as a significant step towards this eventual goal. %We approach the problem from the different angle of learning from first principles, since it is necessary for our purpose. That is, if we want to use machine learning to facilitate the discovery of new algorithms of strong worst-case performance on open problems where we don't have a known difficult input distribution at hand.

\subsection{Summary of results}
%As a brief introduction, we can summarize YaoGANs as essentially starting with a ``random'' algorithm network, then alternating between (1) finding the \emph{best response} (that will force the algorithm to exhibit its worst behavior), and (2) training the algorithm network on this best response. Details are given in \Cref{sec:yaogan}.

We apply the adversarial training to two classic problems in the area of online optimization: the \emph{ski rental} problem and the \emph{AdWords} problem (these are defined formally in \Cref{sec:prelims}). We demonstrate the success of our methods in two ways. Firstly, we show that the \emph{competitive ratio}---the primary figure of quality for an online optimization algorithm---converges to the correct value. To be precise, since it  is not entirely possible to certify the worst-case CR empirically for the more complex problem of AdWords, we show that the learned algorithm achieves near-optimal competitive ratio over learned as well as known hard instances. Secondly, we show that the learned algorithm shares many salient features of the optimal textbook algorithm.

%The two problems exhibit a progression in terms of how hard it is to find the ``best responses.'' Finding best response inputs for ski rental is relatively easy---an approximately exhaustive search (over a suitably parameterized space) is sufficient---while for AdWords it seems to be a hard non-convex global optimization problem.

\textbf{Ski rental.} A typical instance of the ski rental problem is parameterized by multiple parameters, including the size of the input instance $N$. Algorithms accepting only one input size are relatively easier to find than the \emph{uniform algorithms} accepting multiple sizes. We focus on the latter, harder, task by applying proper scaling techniques and best-response learning; such task is beyond the scope of traditional optimization techniques. By applying a straightforward version of adversarial training we recover the optimal textbook uniform algorithm with its behavior matching the one of \cite{Karlin86} with the competitive ratio converging to $1.58$, within $10^{-2}$ of the optimum. We use this concept to demonstrate the effectiveness of the training concept. We include the results on ski rental in the supplementary material.

\textbf{AdWords.}
We solve a fixed-size instance of the fractional Adwords problem---a ``budgeted bipartite matching problem''---with 25 ad slots and 5 advertisers. While learning a uniform algorithm would be preferable, we note that learning how to solve $25 \times 5$ instances is a highly non-trivial task. Using chess or Go as examples, the relevant ML papers solve the games on fixed-size instances rather than on instances of arbitrary size. Of course the latter would be a much stronger result, but the fixed-size task is by no means easy. We use the full end-to-end YaoGAN framework since even finding worst-case inputs in the fractional AdWords is a hard non-convex global optimization problem. Our methods learn an algorithm competitive with the textbook optimal on various input distributions; the learned input instances successfully defeat several reasonable (but non-optimal) approaches like Greedy and the algorithm optimized on a fixed distribution (\Cref{sec:adwords}). Qualitatively, the trained algorithm infers both the \emph{greedy strategy} and the \emph{balance strategy}~\citep{KP00}, two salient properties of the optimal solution. Furthermore, the learned algorithm seems to find the correct trade-off between the strategies in our benchmark.


%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> old_adwords_result.tex <==
%In this section we demonstrate some qualitative behaviors of our training result. We fix $m = 9, n = 3$ and a common budget $B = 3$. We defer the representation details to \Cref{sec:adw-alg-representation} and extra empirical results to \Cref{sec:app-adwords}. About $10$ hours of training is sufficient to achieve a competitive ratio of $\approx 0.7327$, which is within $10^{-2}$ of the theoretically best value achievable for this problem. 

%We start with a brief discussion of the optimal algorithm and input distribution so we can better interpret our results. At a high level, there are two intuitive aspects of the AdWords problem (in the discrete case): the \emph{greedy strategy} and the \emph{balance strategy}. 

%\textbf{Greedy strategy} allocates an ad slot to the advertiser with the highest bid for the ad when their remaining budgets are equal. This is a natural strategy to maximize revenue. %More formally, suppose ad slot $j$ has bids $(v_i)_{i \in [n]}$ at a moment when all advertisers have equal remaining budget. Suppose that for some $i^*$ we have that $v_{i^*} \gg v_{i}\ \forall i \neq i^*$. The MSVV algorithm will completely assign slot $j$ to advertiser $i^*$.

%\textbf{Balance strategy} allocates an ad slot to the advertiser with the largest remaining budget when all advertisers have the same bid for the ad. This is also natural to avoid depleting the budget of any advertiser, since we may run into a future ad where only the advertiser with depleted budget has high bid for the ad. The ``scaled bid" used in the MSVV algorithm (even for the fractional version) can be viewed as a careful interpolation between two strategies when the advertisers' bids and remaining budgets differ. 

%We first demonstrate that our trained algorithm captures the ``greedy" aspect in Figure~\ref{fig:greedy}. For example, in the leftmost plot, we fix the remaining budgets of all advertisers at $2$, the last two advertisers' bid for an ad at $0.25$ (the vertical dotted line), and vary the bid $x$ of advertiser $0$ to plot the fractional allocations returned by the algorithm for different $x$ values. We can see that the algorithm correctly allocates more to advertiser $0$ as the bid $x$ increases, and also correctly allocates roughly the most to the advertiser with the highest bid. We observe consistent behavior for other threshold values in the next $3$ plots (and more comprehensive plots in the appendix).
\begin{figure}[h]
  \begin{center}  
    \includegraphics[width=\textwidth,height=3cm]{figs/Alg_behavior_3x9_weight_short.pdf}
    \caption{Each plot shows the fractional assignment of a new ad to the three different advertisers indexed $\{0, 1, 2 \}$ while keeping the remaining budget equal across all advertisers. The x-axis shows the bid of the first advertiser and the y-axis shows the algorithm agent's fractional assignment $p$.}
    \label{fig:greedy}
  \end{center}
\end{figure}

We demonstrate the ``balance" aspect of our trained algorithm in Figure~\ref{fig:balance}. In the leftmost plot, we vary the remaining budget of advertiser $0$ while fixing the other advertisers' budget at $0.9$, and all advertisers' bids are $1$. The algorithm correctly allocates more the advertiser $0$ when he/she has more remaining budget, and also correctly gives roughly the most fractional share to the advertiser with largest remaining budget. Again, the observation is consistent in the other plots (and more in the appendix).
\begin{figure}[h]
  \begin{center}  
    \includegraphics[width=0.72\textwidth, height=3cm]{figs/Alg_behavior_3x9_budget_a.pdf}
    \caption{Each plot shows the trained agent's allocation of a new ad to three different advertisers indexed $\{0, 1, 2\}$. The ad has a common bid of $1$ from all advertisers. In the $i^{th}$ plot ($i \in \{0, 1, 2\}$) the x-axis denotes the budget of advertiser $i$, while other advertisers have a common remaining budget. The y-axis shows the algorithm agent's fractional assignment $p$.}
    \label{fig:balance}
  \end{center}
\end{figure}
We note that different from the discrete case where one should expect a sharp transition of allocation around the threshold, the smooth curves observed in our plots actually agree with the optimal algorithm in the fractional case. For a concrete example (see Figure~\ref{fig:opt}), we consider the case where the remaining budgets of the advertisers are all fixed at $1$, and advertisers have bids $(x,0.5,0)$ for varying $x$ values. These parameters are chosen for simpler calculation. Let's consider the optimal algorithm's allocation in this case. From our discussion of the optimal fractional algorithm (immediately following the problem definition of fractional AdWords), we know that the optimal algorithm will split the ad between advertiser $0$ and $1$ (as advertiser $2$ has bid $0$), and if the fraction allocated to advertiser $0$ is $t\in [0,1]$, and $1-t$ to advertiser $1$, we must have
\[
x\cdot (1- e^{-\frac{1-t}{3}}) = 0.5\cdot (1- e^{-\frac{1-(1-t)}{3}}) 
\]
If we use the approximation of $e^{-x}\approx 1 -x$ for small $x$, the rough calculation gives $t$ as a function of $x$ where $t=\frac{2x}{2x+1}$. We plot this as the dotted (red) curve in Figure~\ref{fig:opt}, and we observe that the fractional allocation to advertiser $0$ (as a function of $x$) by our trained algorithm is fairly consistent with the optimal.

\begin{figure}[h]
  \begin{center}  
    \includegraphics[width=4cm,height=3cm]{figs/opt_adwords.pdf}
    \caption{The plot shows the trained agent's allocation of a new ad with bids $(x, 0.5, 0)$, where $x$ is the value on the x-axis and y-axis denotes the fractional assignment $p$. All advertisers have a common budget of $1$. The dotted (red) curve depicts the approximate behavior of the optimal algorithm for bidder $0$.}
    \label{fig:opt}
  \end{center}
\end{figure}

On the adversary side, in the specific case of $3$ advertisers and $9$ ad slots, an adversarial input distribution (i.e. a minmax column strategy in the game theoretical discussion of Section~\ref{sec:Yao}) is the uniform distribution over the $6$ matrices which are the column permutations of the transpose of the following matrix, where ads arrive from top to bottom (left-to-right in the transposed matrix below).  
\[
\begin{bmatrix}
    1       & 1 & 1 & 1 & 1& 1& 1& 1& 1\\
    1       & 1 & 1 & 1 & 1& 1 & 0 & 0& 0\\
    1       & 1 & 1 & 0 & 0& 0& 0& 0& 0\\
\end{bmatrix}
\]
In the previous work by~\citet{kong2018new}, they showed that a mixture of an adversarial input distribution and a high-entropy (i.e. noisy) distribution gives a sufficiently good (pre-determined) training set. We plot a set of random samples from the experience array at the end of our training in \Cref{fig:adv} in \Cref{sec:app-adwords}. It is clear that without any expert input, the self-generated input instances during training capture enough structure of such an expert crafted mixture. We find this highly non-trivial. 
%We leave further details to the appendix. 

%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> theory.tex <==
\section{Preliminaries and training framework}\label{sec:prelims}
%We start with a short discussion of online algorithms and give an outline on how adversarial training can be seen through the lens of game theory. We then describe how we implement and stabilize the adversarial training using our ``YaoGAN" framework. 

% \subsection{Online Algorithms and the game-theoretic approach}
% \alert{aranyak: I fear we may just have to drop this game-theory section for space and move CR to intro} In an online problem such as the AdWords or ski-rental, the algorithm has to make an irrevocable decision for each request in the arriving sequence, without knowing the rest of the sequence. 
% %We chose online optimization problems as the testbed for our approach due to their richness in structure and application. 
% %Online problems comprise a theoretical framework to study tasks in the \emph{interactive setting}. In particular, an algorithm agent is given a sequence of requests that require a response without knowing future requests. The full sequence of requests is called an \emph{input instance}. 
% A successful algorithm typically needs to hedge between receiving an immediate reward and allowing for potentially lucrative future rewards.
% The standard measure of the performance of online algorithms is the \emph{competitive ratio} (CR). For a fixed input instance this is the ratio of the (expected) objective value the online algorithm gets for that instance to the \emph{offline optimal value} (the best possible objective value for the instance, knowing the entire sequence upfront). The competitive ratio of the algorithm is defined as its worst competitive ratio over all possible inputs. 
% %Our bottom-line is to \emph{learn algorithms with optimal competitive ratios}. 

% %For readers not familiar with the field of online algorithms \citep{borodin-book}, we include an expanded background discussion in the supplementary material.

% % Appendix~\ref{app:theory}.\alert{GZ: supplementary?}

% One can frame the task of finding an optimal algorithm for a given problem in an abstract game-theoretic setting: Consider a (possibly infinite) two-player zero-sum game matrix $V$, in which
% %we denote the row player as the \emph{algorithm player}, and the column player as the \emph{adversary} who determines the inputs to the algorithm. E
% each row represents a deterministic algorithm $\mc{A}$, and each column represents an input instance $\mc{I}$. The entry $V(\mc{A},\mc{I})$ is the payoff (CR) to Row if it plays $\mc{A}$, and Column player plays $\mc{I}$. 
% %A randomized algorithm is a distribution $\vp$ over rows of $V$; an input distribution $\vq$ is a distribution over columns. In this framing, 
% The worst-case optimal (randomized) algorithm corresponds to Row's max-min strategy. By (von Neumann) strong duality,
% %we see that $\max_{\mc{I}} (\vp^*)^T V(:, \mc{I}) = \min_{\mc{A}} V(\mc{A}, :) \vq^*$, i.e., 
% Column's min-max strategy is therefore the worst (most difficult) input distribution for this problem (this application of duality is called Yao's Lemma~\citep{Yao77} in Theoretical CS). 

% Prior work in~\citep{kong2018new} used this to train an algorithm network on the min-max input distribution for the Adwords problem. Besides the drawback that this needs problem expertise to know the min-max distribution, this approach also has a fatal flaw that Row's best response  to a min-max strategy of Column need not be its own max-min strategy (e.g., in Rock-Paper-Scissors, any pure strategy is a best response to the uniform max-min strategy). Hence, the worst input distribution is not sufficient to recover the best algorithm; this is specifically true for the AdWords problem. Indeed, this issue was acknowledged in~\cite{kong2018new}: they combine multiple types of special input distributions (e.g., universal and high-entropy training sets).
% To overcome this obstacle, we note that solving the game from scratch necessarily requires solving for both the algorithm and the adversary. We draw inspiration from online learning for game-solving \citep{FS96}, and show how we can view adversarial training through the lens of game-theory. Adversarial training intuitively seems to be the ``right thing'' to train algorithms with worst-case guarantees, and we show that the unique challenge now is co-training the Adversary as well, which extends and strengthens the existing adversarial training framework.

%%%%%%%%%%%%%%%%%
%\subsection{Game-theoretic view of robust algorithms}
%\label{sec:Yao}
%\alert{Goran: while I think this section is very important, it might be clear on first reading how it connects to our paper. I'll think about how to make the connection more explicit.}

Consider a (possibly infinite) two-player zero-sum game matrix $V$, where we denote the row player as the \emph{algorithm player}, and the column player as the \emph{adversary} who determines the inputs to the algorithm. Each row represents a deterministic algorithm $\mc{A}$, and each column represents a specific input instance $\mc{I}$, and the corresponding entry $V(\mc{A},\mc{I})$ specifies the payoff to the adversary if the algorithm player plays strategy $\mc{A}$, and the adversary plays strategy $\mc{I}$. We follow the custom that the algorithm player aims to minimize the payoff to the adversary, while the adversary tries to achieve the opposite. In the case of online algorithms, if we are working with a problem with minimization objective, the payoff $V(\mc{A},\mc{I})$ will be the competitive ratio (CR) of $\mc{A}$ for input $\mc{I}$. Similarly, for a maximization problem, we take $V(\mc{A},\mc{I})$ as the negation of the above competitive ratio. We note that general (non-online) algorithmic problems can be cast in the language of two-player zero-sum games as well.

\textbf{Yao's Lemma.} Online algorithms are often randomized since hedging between different input continuations can be elegantly achieved via randomization. %Most notably, in both the ski rental and AdWords problem, \emph{considering only deterministic algorithms significantly lowers the optimal CR}. 
A randomized algorithm can be viewed as a distribution $\vp$ over rows of $V$ (i.e., deterministic algorithms); an input distribution $\vq$ can be viewed as a distribution over columns of $V$ (i.e., input instances). The optimal (potentially randomized) algorithm $\vp^*$ is one whose expected payoff against the worst-case input is minimized, i.e., $\vp^* = \arg\min_{\vp} \max_{\mc{I}} \vp^T V(:,\mc{I})$. A standard result in game-theory stipulates that once you fix a randomized algorithm, then maximizing over pure instances (columns) is equivalent to maximizing over input distributions. The namesake of our paper, Yao's Lemma~\citep{Yao77} says that there exists a distribution $\vq^*$ over inputs such that the expected payoff of the best (deterministic) algorithm over $\vq^*$ is the same as the value of the best randomized algorithm $\vp^*$ over its worst possible (pure) input. In other words, $\max_{\mc{I}} (\vp^*)^T V(:, \mc{I}) = \min_{\mc{A}} V(\mc{A}, :) \vq^*$.  This is, of course, simply an elegant application of von Neumann's minmax theorem aka strong duality to this specific game. Using classic game theory notations, we also refer to the best randomized algorithm as the row player's minmax strategy, and $\vq^*$ the column player's maxmin strategy. Solving an online optimization problem corresponds to solving the above zero-sum game, specifically finding $\vp^*$.

\textbf{Fixed distribution vs. adversarial training.} Most prior work explores algorithmic learning by fixing some input distribution $\vq$ and training only the $\vp$ side. We argue this leads to some major issues in learning robust algorithms. Firstly, we know from basic game theory that optimizing $\vp$ under a fixed $\vq$ converges to a deterministic algorithm, which could be significantly sub-optimal compared to a randomized $\vp^*$ (this is indeed the case in ski rental).
For a simple example, consider the game of rock-paper-scissors. The optimal row strategy is to play the three moves uniformly at random. However, if one fixes the column strategy (e.g., 30\% rock, 40\% paper, 30\% scissors), the optimal response is always a deterministic strategy (e.g., always play scissors). Secondly, even if the optimal algorithm is deterministic (as in AdWords), there is no guarantee that it can be found as the optimal response to a fixed distribution of inputs. In fact, if we were to train against the fixed $\vq^*$, there may be other best responses besides $\vp^*$. In rock-paper-scissors, any row (and any mixed row strategy) is a best response to the maxmin column strategy $(1/3, 1/3, 1/3)$. This issue has been acknowledged in~\cite{kong2018new}: they combine multiple types of special input distributions (e.g., universal and high-entropy training sets) and use the implicit regularization of reinforcement learning to train robust algorithms. 
%The maxmin column strategy is to play the three moves uniformly at random, and any row strategy (e.g., always play rock) is a best response to the column player's minmax strategy. %Thus, training the algorithm network on the adversarial distribution by itself does not necessarily guarantee obtaining the optimal algorithm. 
%Indeed, this was acknowledged in~\citet{kong2018new}, e.g., for the AdWords problem they combined the adversarial distribution with another hand-picked input distribution to avoid converging to a suboptimal greedy algorithm. 
%They address the $\vq^*$ by considering only problems for which the optimal input distribution is known. However, there are two acknowledged weaknesses in this approach:

%problems where such a distribution is known, prior work~\citep{kong2018new} has exploited this idea to find theoretically optimal algorithms for online optimization problems. However, there are two acknowledged weaknesses in this approach:

%First, such knowledge of the adversarial maxmin distribution is typically only available for well-studied problems where we already have a theoretically established limit on the performance of any algorithm. Thus, to fulfill the ultimate goal of using machine learning to discover (unknown) algorithms with competitive ``worst-case" performances, we need an approach without relying on domain knowledge of a worst-case input distribution. 

%Second, a somewhat fundamental issue with the approach is that an algorithm that performs well against the adversarial distribution alone is in fact not necessarily the optimal algorithm. %Consider the zero-sum game described above. We are interested in finding the optimal algorithm (i.e., minmax strategy for the case of minimization problems) for the row player. The adversarial input distribution is a known maxmin strategy for the column player. However, it is not the case, in general, that the only best response to a maxmin strategy is a minmax strategy.
%For a simple example, consider the game of rock-paper-scissors. The maxmin column strategy is to play the three moves uniformly at random, and any row strategy (e.g., always play rock) is a best response to the column player's minmax strategy. %Thus, training the algorithm network on the adversarial distribution by itself does not necessarily guarantee obtaining the optimal algorithm. 
%Indeed, this was acknowledged in~\citet{kong2018new}, e.g., for the AdWords problem they combined the adversarial distribution with another hand-picked input distribution to avoid converging to a suboptimal greedy algorithm. 

Indeed, solving the game requires co-training both the row (algorithm) and column (input) sides. Adversarial training seems to be the ``right thing'' to train algorithms with worst-case guarantees, and the unique challenge in our case requires co-training the Adversary as well, which extends and strengthens the existing adversarial training framework. We note in \Cref{sec:adwords} that training an algorithm via YaoGAN is appears significantly easier than with previous fixed-distribution approaches. Furthermore, we give an indirect theoretical justification for the power of adversarial learning for solving zero-sum games using no-regret dynamics (see supplementary material).

% \subsection{AdWords}\label{sec:def-adwords}

% We formally define the {\bf AdWords} problem~\citep{MSVV07}: There are $m$ advertisers with budget $B$ each, and $n$ ad slots. Each ad slot $j$ arrives sequentially along with a vector $v^j = (v^j_0, v^j_2, \ldots, v^j_{m-1})$ where $v^j_{i}$ is the bid of advertiser $i$ for slot $j$. Once a slot arrives the algorithm must irrevocably be allocated to an advertiser or no one at all. In the event that the ad $j$ is allocated to advertiser $i$, the algorithm collects a revenue which is the minimum of $v^j_i$ and advertiser $i$'s remaining budget. The remaining budget of advertiser $i$ is reduced accordingly. The objective of the algorithm is to maximize the total revenue over the entire sequence.

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

